MFIT: Multi-Fidelity Thermal Modeling for 2.5D and 3D Multi-Chiplet Architectures

Rapidly evolving artificial intelligence and machine learning applications require ever-increasing computational capabilities, while monolithic 2D design technologies approach their limits. Heterogeneous integration of smaller chiplets using a 2.5D silicon interposer and 3D packaging has emerged as a promising paradigm to address this limit and meet performance demands. These approaches offer a significant cost reduction and higher manufacturing yield than monolithic 2D integrated circuits. However, the compact arrangement and high compute density exacerbate the thermal management challenges, potentially compromising performance. Addressing these thermal modeling challenges is critical, especially as system sizes grow and different design stages require varying levels of accuracy and speed. Since no single thermal modeling technique meets all these needs, this paper introduces MFIT, a range of multi-fidelity thermal models that effectively balance accuracy and speed. These multi-fidelity models can enable efficient design space exploration and runtime thermal management. Our extensive testing on systems with 16, 36, and 64 2.5D integrated chiplets and 16x3 3D integrated chiplets demonstrates that these models can reduce execution times from days to mere seconds and milliseconds with negligible loss in accuracy.

==> files/accuracy_table_2.5D.tex <==
\begin{table*}[ht]
    %\vspace{-8pt}
    \caption{Mean Absolute Error and accuracy in predicting temperature violations are shown as compared to reference FEM results. The thermal RC, DSS, and HotSpot~\cite{skadron_temperatureAware} models are shown.}
    %\vspace{-8pt}
    % \footnotesize
    \centering
    \renewcommand{\arraystretch}{0.9}
    \begin{subtable}{0.4\linewidth}
    %\vspace{-4pt}
    \subcaption{16 Chiplets}
    %\vspace{-4pt}
        \begin{tabular}{@{}cc|cc@{}}
        \toprule
        \textbf{} & \textbf{} & \textbf{MAE ($^{\circ}$C)} & \textbf{\begin{tabular}[c]{@{}c@{}} Temp. violation \\ accuracy(\%) \end{tabular} }\\ \midrule
        \multirow{3}{*}{WL1} & Thermal RC & 1.23 & \highlight{93.4} \\
         & DSS & 1.23 & \highlight{93.4} \\ 
         & \textit{HotSpot} & \textit{2.74} & \textit{67.7} \\ \midrule
        \multirow{3}{*}{WL2} & Thermal RC & 0.86 & 95.9 \\
         & DSS & 0.86 & 95.9 \\ 
         & \textit{HotSpot} & \textit{1.57} & \textit{75.0}\\ \midrule
        \multirow{3}{*}{WL3} & Thermal RC & 1.02 & 100 \\
         & DSS & 1.02 & 100 \\ 
         & \textit{HotSpot} & \textit{1.97} &  \textit{100}\\ \midrule
        \multirow{3}{*}{WL4} & Thermal RC & \highlight{1.41} & 96.6 \\
         & DSS & \highlight{1.41} & 96.6 \\ 
         & \textit{HotSpot} & \textit{2.29} & \textit{95.6}\\ \midrule
        \multirow{3}{*}{WL5} & Thermal RC & 1.01 & 100 \\
         & DSS & 1.01 & 100 \\ 
         & \textit{HotSpot} & \textit{1.94} & \textit{100}\\ \midrule
        \multirow{3}{*}{WL6} & Thermal RC & 0.89 & 98.1 \\
         & DSS & 0.89 & 98.1 \\ 
         & \textit{HotSpot} &\textit{1.62}& \textit{85.8}\\
        \bottomrule
    \end{tabular}
    \end{subtable}
    \hspace{-0.05\linewidth}
    \begin{subtable}{0.25\linewidth}
    %\vspace{-4pt}
    \subcaption{36 chiplets}
    %\vspace{-4pt}
    \centering
        \begin{tabular}{cc}
        \toprule
        \textbf{MAE ($^{\circ}$C)} & \textbf{\begin{tabular}[c]{@{}c@{}} Temp. violation \\ accuracy(\%) \end{tabular} } \\ \midrule
         1.42 & 96.9 \\%wl1
         1.42 & 96.9 \\ 
         \textit{1.64} & \textit{96.9} \\ \midrule
         1.16 & 100 \\%wl2
         1.16 & 100 \\ 
         \textit{1.24} & \textit{100} \\ \midrule
         1.28 & \highlight{77.2} \\%wl3
         1.28 & \highlight{77.2} \\ 
         \textit{1.18} & \textit{42.3} \\ \midrule
         \highlight{1.63} & 95.5 \\%wl4
         \highlight{1.63} & 95.5 \\ 
         \textit{1.89} & \textit{92.0} \\ \midrule
         1.25 & 87.8 \\%wl5
         1.25 & 87.8 \\ 
         \textit{1.16} & \textit{60.7} \\ \midrule
         1.30 & 84.8 \\%wl6
         1.30 & 84.8 \\ 
         \textit{1.28} & \textit{89.7} \\ 
        \bottomrule
    \end{tabular}
    \end{subtable}
    \hspace{-0.02\linewidth}
    \begin{subtable}{0.25\linewidth}
    %\vspace{-4pt}
    \subcaption{64 chiplets}
    %\vspace{-4pt}
    \centering
        \begin{tabular}{cc}
        \toprule
        \textbf{MAE ($^{\circ}$C)} & \textbf{\begin{tabular}[c]{@{}c@{}} Temp. violation \\ accuracy(\%) \end{tabular} } \\ \midrule
         1.17 & 99.2 \\%wl1
         1.17 & 99.2 \\ 
         \textit{1.69} & \textit{98.1} \\ \midrule
         1.08 & 100 \\%wl2
         1.08 & 100 \\ 
         \textit{1.19} & \textit{100} \\ \midrule
         1.17 & 89.3 \\%wl3
         1.17 & 89.3 \\ 
         \textit{1.33} & \textit{74.4} \\ \midrule
         \highlight{1.55} & 97.6 \\%wl4
         \highlight{1.55} & 97.6 \\ 
         \textit{2.15} & \textit{97.7} \\ \midrule
         1.07 & \highlight{82.4} \\%wl5
         1.07 & \highlight{82.4} \\ 
         1.40 & 52.9 \\ \midrule
         1.21 & 90.9 \\%wl6
         1.21 & 90.9 \\ 
         \textit{1.56} & \textit{89.5} \\ 
        \bottomrule
    \end{tabular}
    \end{subtable}
    % %\vspace{-10pt}


        \begin{subtable}{0.25\linewidth}
    %\vspace{-4pt}
    \subcaption{64 chiplets}
    %\vspace{-4pt}
    \centering
        \begin{tabular}{cc}
        \toprule
        \textbf{MAE ($^{\circ}$C)} & \textbf{\begin{tabular}[c]{@{}c@{}} Temp. violation \\ accuracy(\%) \end{tabular} } \\ \midrule
         1.17 & 99.2 \\%wl1
         1.17 & 99.2 \\ 
         \textit{1.69} & \textit{98.1} \\ \midrule
         1.08 & 100 \\%wl2
         1.08 & 100 \\ 
         \textit{1.19} & \textit{100} \\ \midrule
         1.17 & 89.3 \\%wl3
         1.17 & 89.3 \\ 
         \textit{1.33} & \textit{74.4} \\ \midrule
         \highlight{1.55} & 97.6 \\%wl4
         \highlight{1.55} & 97.6 \\ 
         \textit{2.15} & \textit{97.7} \\ \midrule
         1.07 & \highlight{82.4} \\%wl5
         1.07 & \highlight{82.4} \\ 
         1.40 & 52.9 \\ \midrule
         1.21 & 90.9 \\%wl6
         1.21 & 90.9 \\ 
         \textit{1.56} & \textit{89.5} \\ 
        \bottomrule
    \end{tabular}
    \end{subtable}
    
    \label{tab:chiplet_accuracy}
\end{table*}


==> files/accuracy_table_3D.tex <==
\begin{table}[ht]
    % \vspace{-8pt}
    \caption{Mean Absolute Error and accuracy in predicting temperature violations are shown as compared to reference FEM results for a 3D 48 chiplet system. The thermal RC, DSS, and HotSpot~\cite{skadron_temperatureAware} models are shown.}
    % \vspace{-8pt}
    % \footnotesize
    % \renewcommand{\arraystretch}{0.9}
    % \vspace{-4pt}
    \centering
    \begin{tabular}{@{}cc|cc@{}}
        \toprule
        \textbf{} & \textbf{} & \textbf{MAE ($^{\circ}$C)} & \textbf{\begin{tabular}[c]{@{}c@{}} Temp. violation \\ accuracy(\%) \end{tabular} }\\ \midrule
        \multirow{3}{*}{WL1} & Thermal RC & 0.82 & 99.7 \\
         & DSS & 0.82 & 99.7 \\ 
         & \textit{HotSpot} & \textit{1.32} &  \textit{94.5}\\ \midrule
         
         \multirow{3}{*}{WL2} & Thermal RC & 1.08 & 100 \\
         & DSS & 1.08 & 100 \\ 
         & \textit{HotSpot} & \textit{1.19} & \textit{100} \\ \midrule
         
         \multirow{3}{*}{WL3} & Thermal RC & 1.05 & 100 \\
         & DSS & 1.05 & 100 \\ 
         & \textit{HotSpot} & \textit{1.08} & \textit{100}\\ \midrule
        
        \multirow{3}{*}{WL4} & Thermal RC & \highlight{1.30} & 99.3 \\
         & DSS & \highlight{1.30} & 99.3 \\ 
         & \textit{HotSpot} & \textit{1.85} & \textit{98.0}\\ \midrule
         
         \multirow{3}{*}{WL5} & Thermal RC & 1.03 & 100 \\
         & DSS & 1.03 & 100 \\ 
         & \textit{HotSpot} &\textit{1.05}& \textit{100}\\ \midrule

        \multirow{3}{*}{WL6} & Thermal RC & 1.11 & \highlight{98.3} \\
         & DSS & 1.11 & \highlight{98.3} \\ 
         & \textit{HotSpot} & \textit{1.24} & \textit{86.7}\\ 
        
        \bottomrule
    \end{tabular}
    % \vspace{-10pt}
    \label{tab:3D_accuracy}
\end{table}


==> temp.tex <==
\begin{table*}[ht]
    \caption{Mean Absolute Error and accuracy in predicting temperature violations are shown as compared to reference FEM results. The thermal RC, DSS, HotSpot~\cite{skadron_temperatureAware}, 3D-ICE\cite{3D_ICE}, and PACT \cite{pact} models are shown. Best MAE for each system-workload combination are highlighted in red. \textbf{Average operating temperatures are in the range of 60-80 ($^\circ$C).}}
    \centering
    % \renewcommand{\arraystretch}{0.98}
    \setlength{\tabcolsep}{2pt} % Adjust column separation
    \scriptsize % Reduce font size to fit the table on the page

    % Begin the tabular environment with appropriate column definitions
    \begin{tabular}{@{}ll|ccc|ccc|ccc|ccc@{}}
        \toprule
        % First row: Headers for each section
        \multicolumn{2}{c|}{} & \multicolumn{3}{c|}{\textbf{2.5D - 16 Chiplets}} & \multicolumn{3}{c|}{\textbf{2.5D - 36 Chiplets}} & \multicolumn{3}{c|}{\textbf{2.5D - 64 Chiplets}} & \multicolumn{3}{c}{\textbf{3D - 16x3 Chiplets}} \\ \midrule

        % Second row: Sub-headers for each section
        \textbf{Workload} & \textbf{Model} & \textbf{MAE & \textbf{\begin{tabular}[c]{@{}c@{}}Avg. \%\\ Error\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Temp. Violation\\Accuracy\end{tabular}} &
        \textbf{MAE}  & \textbf{\begin{tabular}[c]{@{}c@{}}Avg. \%\\ Error\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Temp. Violation\\Accuracy\end{tabular}} &
        \textbf{MAE} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg. \%\\ Error\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Temp. Violation\\Accuracy\end{tabular}} &
        \textbf{MAE}  & \textbf{\begin{tabular}[c]{@{}c@{}}Avg. \%\\ Error\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Temp. Violation\\Accuracy\end{tabular}} \\ \midrule
        \multirow{5}{*}{WL1} & Thermal RC & \highlight{1.23$^\circ$C} & & 93.5 & \highlight{1.42$^\circ$C} & 96.9 & \highlight{0.99$^\circ$C} & 100.0 & \highlight{0.94$^\circ$C} & 98.1 \\
        & DSS & \highlight{1.23$^\circ$C} & 93.5 & \highlight{1.42$^\circ$C} & 96.9 & \highlight{0.99$^\circ$C} & 100.0 & \highlight{0.94$^\circ$C} & 98.1 \\
        & \textit{HotSpot} & 2.74$^\circ$C & 67.8 & 1.64$^\circ$C & 97.0 & 2.16$^\circ$C & 96.9 & 2.37$^\circ$C & 87.6 \\
        & \textit{3D-ICE} & 1.65$^\circ$C & 89.5 & 2.07$^\circ$C & 98.0 & 1.65$^\circ$C & 99.6 & 1.73$^\circ$C & 97.7 \\
        & \textit{PACT} & 1.99$^\circ$C & 91.7 & 1.61$^\circ$C & 99.2 & 1.70$^\circ$C & 99.4 & 2.09$^\circ$C & 99.0 \\
        \midrule
        \multirow{5}{*}{WL2} & Thermal RC & \highlight{0.86$^\circ$C} & 96.0 & 1.16$^\circ$C & 78.48 & \highlight{0.95$^\circ$C} & 95.83 & \highlight{0.98$^\circ$C} & 100.0 \\
        & DSS & \highlight{0.86$^\circ$C} & 96.0 & 1.16$^\circ$C & 78.48 & \highlight{0.95$^\circ$C} & 95.83 & \highlight{0.98$^\circ$C} & 100.0 \\
        & \textit{HotSpot} & 1.58$^\circ$C & 75.0 & 1.24$^\circ$C & 29.74 & 1.01$^\circ$C & 67.36 & 1.74$^\circ$C & 100.0 \\
        & \textit{3D-ICE} & 1.36$^\circ$C & 85.1 & 1.35$^\circ$C & 3.79 & 1.82$^\circ$C & 76.38 & 1.39$^\circ$C & 100.0 \\
        & \textit{PACT} & 1.58$^\circ$C & 75.9 & \highlight{0.91$^\circ$C} & 23.41 & 1.55$^\circ$C & 66.66 & 2.10$^\circ$C & 100.0 \\
        \midrule
        \multirow{5}{*}{WL3} & Thermal RC & \highlight{1.02$^\circ$C} & 100.0 & 1.28$^\circ$C & 77.3 & \highlight{1.03$^\circ$C} & 97.0 & \highlight{0.80$^\circ$C} & 100.0 \\
        & DSS & \highlight{1.02$^\circ$C} & 100.0 & 1.28$^\circ$C & 77.3 & \highlight{1.03$^\circ$C} & 97.0 & \highlight{0.80$^\circ$C} & 100.0 \\
        & \textit{HotSpot} & 1.97$^\circ$C & 100.0 & 1.18$^\circ$C & 42.4 & 1.12$^\circ$C & 72.3 & 1.79$^\circ$C & 100.0 \\
        & \textit{3D-ICE} & 1.15$^\circ$C & 100.0 & 1.53$^\circ$C & 14.9 & 1.82$^\circ$C & 80.7 & 1.12$^\circ$C & 100.0 \\
        & \textit{PACT} & 2.03$^\circ$C & 100.0 & \highlight{1.09$^\circ$C} & 42.4 & 1.75$^\circ$C & 72.3 & 1.80$^\circ$C & 100.0 \\
        \midrule
        \multirow{5}{*}{WL4} & Thermal RC & \highlight{1.46$^\circ$C} & 96.6 & \highlight{1.64$^\circ$C} & 95.6 & \highlight{1.35$^\circ$C} & 96.8 & \highlight{1.48$^\circ$C} & 98.5 \\
        & DSS & \highlight{1.46$^\circ$C} & 96.6 & \highlight{1.64$^\circ$C} & 95.6 & \highlight{1.35$^\circ$C} & 96.8 & \highlight{1.48$^\circ$C} & 98.5 \\
        & \textit{HotSpot} & 2.29$^\circ$C & 95.6 & 7.39$^\circ$C & 92.0 & 2.10$^\circ$C & 96.5 & 2.71$^\circ$C & 96.7 \\
        & \textit{3D-ICE} & 3.72$^\circ$C & 91.3 & 2.33$^\circ$C & 97.0 & 2.68$^\circ$C & 97.4 & 2.46$^\circ$C & 96.8 \\
        & \textit{PACT} & 3.56$^\circ$C & 93.8 & 1.94$^\circ$C & 97.7 & 2.39$^\circ$C & 97.4 & 2.97$^\circ$C & 96.6 \\
        \midrule
        \multirow{5}{*}{WL5} & Thermal RC & \highlight{1.01$^\circ$C} & 100.0 & 1.25$^\circ$C & 87.9 & \highlight{0.96$^\circ$C} & 82.9 & \highlight{0.87$^\circ$C} & 100.0 \\
        & DSS & \highlight{1.01$^\circ$C} & 100.0 & 1.25$^\circ$C & 87.9 & \highlight{0.96$^\circ$C} & 82.9 & \highlight{0.87$^\circ$C} & 100.0 \\
        & \textit{HotSpot} & 1.95$^\circ$C & 100.0 & 1.16$^\circ$C & 60.7 & 1.30$^\circ$C & 2.9 & 1.86$^\circ$C & 100.0 \\
        & \textit{3D-ICE} & 1.16$^\circ$C & 100.0 & 1.53$^\circ$C & 20.0 & 1.79$^\circ$C & 48.6 & \highlight{0.87$^\circ$C} & 100.0 \\
        & \textit{PACT} & 1.99$^\circ$C & 100.0 & \highlight{1.13$^\circ$C} & 53.2 & 1.87$^\circ$C & 17.1 & 1.64$^\circ$C & 100.0 \\
        \midrule
        \multirow{5}{*}{WL6} & Thermal RC & \highlight{0.89$^\circ$C} & 98.1 & 1.30$^\circ$C & 84.8 & \highlight{1.21$^\circ$C} & 92.8 & \highlight{1.52$^\circ$C} & 94.0 \\
        & DSS & \highlight{0.89$^\circ$C} & 98.1 & 1.30$^\circ$C & 84.8 & \highlight{1.21$^\circ$C} & 92.8 & \highlight{1.52$^\circ$C} & 94.0 \\
        & \textit{HotSpot} & 1.62$^\circ$C & 85.9 & \highlight{1.28$^\circ$C} & 89.8 & 1.48$^\circ$C & 77.2 & 2.22$^\circ$C & 81.4 \\
        & \textit{3D-ICE} & 1.34$^\circ$C & 91.8 & 1.69$^\circ$C & 78.5 & 2.38$^\circ$C & 76.2 & 1.61$^\circ$C & 74.9 \\
        & \textit{PACT} & 1.67$^\circ$C & 89.3 & 1.28$^\circ$C & 91.7 & 1.85$^\circ$C & 92.8 & 2.43$^\circ$C & 69.8 \\
        \bottomrule
    \end{tabular}
    \label{tab:combined_accuracy}
\end{table*}

